Efficient Least Residual Greedy Algorithms for Sparse Recovery

We present a novel stagewise strategy for improving greedy algorithms for sparse recovery. We demonstrate its efficiency both for synthesis and analysis sparse priors, where in both cases we demonstrate its computational efficiency and competitive reconstruction accuracy. In the synthesis case, we also provide theoretical guarantees for the signal recovery that are on par with the existing perfect reconstruction bounds for the relaxation-based solvers and other sophisticated greedy algorithms.

==> commands.tex <==
%\usepackage{nohyperref}
% if you need to pass options to natbib, use, e.g.:
% \PassOptionsToPackage{numbers, compress}{natbib}
% before loading nips_2016
%
% to avoid loading the natbib package, add option nonatbib:
% \usepackage[nonatbib]{nips_2016}
%\usepackage[sort&compress]{natbib}

%\usepackage{guidelines/nips_2016}

% to compile a camera-ready version, add the [final] option, e.g.:
%\usepackage[final]{guidelines/nips_2016}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage[bookmarks=false]{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage[firstinits=true,natbib=true]{biblatex}
%\bibliography{paper_refs}
\usepackage{bm}
\usepackage{esvect}
\usepackage[rgb]{xcolor}
%\usepackage{pdfcomment}
\usepackage{amsthm}
\usepackage{etoolbox}
\usepackage{multicol}
\usepackage{scrextend}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{placeins}
\usepackage{caption}
\usepackage{listings}
\usepackage{textgreek}


%\usepackage{titling}
\captionsetup[table]{name=Algorithm}
%\usepackage{cite}

%\makeatletter
%\patchcmd{\@cmidrulea}{\hfill}{\hfill\kern\z@}{}{}
%\patchcmd{\@cmidruleb}{\hfill}{\hfill\kern\z@}{}{}
%\makeatother


\newcommand{\HL}[1]{\pdfmarkupcomment[markup=Highlight,color=yellow]{#1}{#1}}
\newcommand{\HC}[2]{\pdfmarkupcomment[markup=Highlight,color=green]{#1}{#2}}
\newcommand{\HQ}[1]{\pdfmarkupcomment[markup=Highlight,color=pink]{?}{#1}}


%	}
%\makeatletter
%\def\HL{\@ifnextchar[{\@HLwithcomment}{\@HLwithoutcomment}}
%\def\@HLwithcomment[#1]#2{\pdfmarkupcomment[markup=Highlight,author=GL]{#2}{highlighted text - #1}}
%\def\@HLwithoutcomment#1{\pdfmarkupcomment[markup=Highlight,author=GL]{#1}{highlighted text}}
%\makeatother

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{prob}{Problem}[section] 
\newdefinition{df}{Definition}
\newdefinition{rmk}{Remark}
\newproof{prf}{Proof}



\newcommand{\OOO}{\mathcal{O}}
\newcommand{\NNN}{\mathcal{N}}
\newcommand\Aa{\arraycolsep=1.4pt\left[\begin{array}{cc}\mA&\va\end{array}\right]}

\newcommand\Aia{\arraycolsep=1.4pt\left[\begin{array}{cc}\Ai&\va\end{array}\right]}
\newcommand\Aat{\left[\begin{array}{c}\mA^T\\\va^T\end{array}\right]}
\newcommand\errt{\ensuremath\widetilde{err}}
\newcommand\Bt{\tilde{\mB}}
\newcommand\BZZZ{\left[ \begin{array}{cc} \mB & 0 \\ 0 & 0 \end{array} \right]}
\newcommand{\norms}[1]{\left\Vert#1\right\Vert^2}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}
\newcommand{\ips}[1]{\langle #1 \rangle}
\newcommand\gt[2]{\tabto{#1}($#2$)}
\newcommand\Ai{\mA_{\setminus i}}
\newcommand\Aj{\mA_{\setminus j}}
\newcommand\Ak{\mA_{\setminus k}}
\newcommand\Bi{\mB_{\setminus i}}
\newcommand\Bii{\mB_{\setminus i, \mi}}
\newcommand\Aij{\mA_{\setminus i,j}}
\newcommand\Ri{R_{\mA_{\setminus i}}}
\newcommand\Rj{R_{\sTj}}
%\newcommand\Rij{R_{\mA_{\setminus i,j}}}
\newcommand\Lt{\tilde{\sL}} 
\newcommand\Tt{\tilde{\sT}} 
\newcommand\yt{\tilde{\vec{y}}} 
\newcommand\xt{\tilde{\vec{x}}} 
\newcommand\xh{\hat{\vec x}} 
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand\At{{\tilde{\mA}}}
\newcommand\Atk{{\tilde{\mA}_{\setminus k}}}
\newcommand{\mi}{{\setminus i}}
\newcommand\BZZZi{\left[ \begin{array}{cc} \Bi & 0 \\ 0 & 0 \end{array} \right]}





\newcommand\vrho{\vec{\rho}}
\newcommand\vy{\vec{y}}
\newcommand\vc{\vec{c}}
\newcommand\va{\vec{a}}
\newcommand\vr{\vec{r}}
\newcommand\vz{\vec{z}}
\newcommand{\di}{\vd_{(i)}}
\renewcommand{\dj}{\vd_{(j)}}
\newcommand{\vo}{\vec{\omega}}
\newcommand{\oi}{\vo_{(i)}}
\newcommand{\oj}{\vo_{(j)}}
\newcommand{\vd}{\vec{d}}
\newcommand\vw{\vec{w}}
\newcommand\vx{\vec{x}}
\newcommand\ve{\vec{e}}
\newcommand{\vb}{\vec{b}}
\newcommand{\vu}{\vec{u}}
\renewcommand{\v}{\vec{v}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vg}{\vec{g}}
\newcommand{\valpha}{{\vec{\alpha}}}
%\newcommand{\valphai}{{\valpha_i}}
%\newcommand{\valphaj}{{\valpha_j}}
\newcommand{\vgam}{\vec{\gamma}}
\newcommand\sett[1]{{#1}}
\newcommand{\sT}{{\sett{T}}}
\newcommand{\sTt}{{\sett{T}\cup i }}
\newcommand{\sTj}{{\sett{T}\setminus j }}
\newcommand{\sL}{{\sett{L}}}
\newcommand{\sS}{{\sett{S}}}
\newcommand{\sLam}{{\sett{\Lambda}}}
\newcommand{\sLami}{{\sLam \cup i}}
\newcommand{\sLammi}{{\sLam \setminus i}}
\newcommand{\sLamz}{{\sLam_0}}
\newcommand{\sLamzc}{{\sLam_0^c}}



\newcommand{\matrx}[1]{\bm{#1}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\mA}{{\matrx{A}}}
\newcommand{\mB}{{\matrx{B}}}
\newcommand{\mD}{{\matrx{D}}}
\newcommand{\mI}{{\matrx{I}}}
\newcommand{\mM}{\matrx{M}}
\newcommand{\mC}{\matrx{C}}
\newcommand{\mO}{\matrx{\Omega}}
\newcommand{\mQ}{\matrx{Q}}
\newcommand{\QM}{\mQ_{\mM}}
\newcommand{\QO}{\mQ_{\mM^\perp}}
\newcommand{\OL}{\mO_\sLam}
\newcommand{\OLi}{\mO_\sLami}
\newcommand{\OLmi}{\mO_\sLammi}
\newcommand{\BL}{\mB_\Lambda^{-1}}
\newcommand{\CL}{\mC_\Lambda}
\newcommand{\Zer}{\matrx{0}}
\newcommand{\mL}{\matrx{L}}
\newcommand{\LL}{\mL_\Lambda}
\newcommand{\mJ}{\matrx{J}}
\newcommand{\mK}{\matrx{K}}


\newcommand{\Rn}{R_{\sT_n}}
\newcommand{\Rnn}{R_{\sT_{n+1}}}
\newcommand{\Pn}{P_{\sT_n}}
\newcommand{\Pnn}{P_{\sT_{n+1}}}

\newcommand{\MMM}[2]{\left[\begin{array}{#1} #2 \end{array}\right]} 


\newcommand{\ORIP}{$\Omega$-RIP\xspace}
\newcommand{\deltaO}{\delta^\Omega} 
\newcommand{\deltaD}{\delta^D} 
 




\newcommand{\cosamp}{CoSaMP\xspace}
%\newcommand{\vs}{\vspace{-0.1cm}}



\newcommand{\vs}{}
\numberwithin{equation}{section}
\numberwithin{df}{section}

	%\setlength\abovedisplayshortskip
	
	
	\expandafter\def\expandafter\normalsize\expandafter{%
		\normalsize
	\setlength\abovedisplayskip{5.0pt plus 2.0pt minus 3.0pt}
	\setlength\belowdisplayskip{5.0pt plus 2.0pt minus 3.0pt}
	\setlength\belowdisplayshortskip{3.0pt plus 2.0pt minus 2.0pt}
}


